Bound and Conquer: Improving Triangulation by Enforcing Consistency

We study the accuracy of triangulation in multi-camera systems with respect to the number of cameras. We show that, under certain conditions, the optimal achievable reconstruction error decays quadratically as more cameras are added to the system. Furthermore, we analyse the error decay-rate of major state-of-the-art algorithms with respect to the number of cameras. To this end, we introduce the notion of consistency for triangulation, and show that consistent reconstruction algorithms achieve the optimal quadratic decay, which is asymptotically faster than some other methods. Finally, we present simulations results supporting our findings. Our simulations have been implemented in MATLAB and the resulting code is available in the supplementary material.

==> chapters/backup.tex <==
\subsection{2-D linear camera array}
\input{./figures/plot_synthesised_2D.tex}

We first perform a simulation of a linear camera array in $2$-D, assuming pixelisation is the only source of uncertainty. In this case, the $2$-D world is split into a finite number of consistent regions, each corresponding to a unique feature trajectory. This allows the expected reconstruction error to be calculated as a sum of integrals, one over each consistent region. These integrals can be easily approximated using standard numerical techniques.

Another advantage of the $2$-D case is that we can use a brute force strategy to find the globally optimal $\ell_2$ and $\ell_\infty$ reconstructions. The resulting error decays are depicted in Fig. \ref{fig_lincamquadgrowth_logscale}. Here, the region of interest has been defined as the union of all finite-size consistent regions and for computational reasons, each camera has just five pixels. Although this setup is very artificial, we can clearly see the quadratic error decay of the $\ell_\infty$-norm  (its slope is $-2$ on the log-log plot). Similarly, linear triangulation has a linear error decay (slope of $-1$) and the $\ell_2$-norm starts off quadratic but breaks down at $M=14$. This break down occurs because the $\ell_2$-approach fails to return consistent estimates as the number of cameras increase.

To show that the breakdown of the $\ell_2$ approach is not a problem with the brute force search, we added a fourth algorithm, which we call consistent min. $\ell_2$-norm. For this algorithm, we return the point in the consistent region that has minimum $\ell_2$-norm. As is clear from the figure, this approach also achieves the quadratic decay, as expected. In addition, we verified that the $\ell_2$-norm of the point selected by the brute force search was indeed less than the minimum inside the consistent region (unless it was the same point). 
